Accurate Molecular Dynamics Enabled by Efficient Physically-Constrained Machine Learning Approaches

We develop a combined machine learning (ML) and quantum mechanics approach that enables data-efficient reconstruction of flexible molecular force fields from high-level ab initio calculations, through the consideration of fundamental physical constraints. We discuss how such constraints are recovered and incorporated into ML models. Specifically, we use conservation of energy - a fundamental property of closed classical and quantum mechanical systems -- to derive an efficient gradient-domain machine learning (GDML) model. The challenge of constructing conservative force fields is accomplished by learning in a Hilbert space of vector-valued functions that obey the law of energy conservation. We proceed with the development of a multi-partite matching algorithm that enables a fully automated recovery of physically relevant point-group and fluxional symmetries from the training dataset into a symmetric variant of our model. The developed symmetric GDML (sGDML) approach is able to faithfully reproduce global force fields at the accuracy high-level ab initio methods, thus enabling sample intensive tasks like molecular dynamics simulations at that level of accuracy.

==> referenc.tex <==
\begin{thebibliography}{100}

\bibitem{poltavsky2016modeling}
Igor Poltavsky and Alexandre Tkatchenko.
\newblock Modeling quantum nuclei with perturbed path integral molecular
  dynamics.
\newblock {\em Chem. Sci.}, 7(2):1368--1372, 2016.

\bibitem{vanderMaaten2008}
Laurens van~der Maaten and Geoffrey Hinton.
\newblock Visualizing data using {t-SNE}.
\newblock {\em J. Mach. Learn. Res.}, 9(2579-2605):85, 2008.

\bibitem{AMBER1981}
Paul~K. Weiner and Peter~A. Kollman.
\newblock {AMBER}: {A}ssisted model building with energy refinement. {A}
  general program for modeling molecules and their interactions.
\newblock {\em J. Comput. Chem.}, 2(3):287--303, 1981.

\bibitem{amber18}
D.A. Case, I.Y. Ben-Shalom, S.R. Brozell, D.S. Cerutti, T.E. {Cheatham, III},
  V.W.D. Cruzeiro, T.A. Darden, R.E. Duke, D.~Ghoreishi, M.K. Gilson,
  H.~Gohlke, A.W. Goetz, D.~Greene, R~Harris, N.~Homeyer, S.~Izadi,
  A.~Kovalenko, T.~Kurtzman, T.S. Lee, S.~LeGrand, P.~Li, C.~Lin, J.~Liu,
  T.~Luchko, R.~Luo, D.J. Mermelstein, K.M. Merz, Y.~Miao, G.~Monard,
  C.~Nguyen, H.~Nguyen, I.~Omelyan, A.~Onufriev, F.~Pan, R.~Qi, D.R. Roe,
  A.~Roitberg, C.~Sagui, S.~Schott-Verdugo, J.~Shen, C.L. Simmerling, J.~Smith,
  R.~Salomon-Ferrer, J.~Swails, R.C. Walker, J.~Wang, H.~Wei, R.M. Wolf, X.~Wu,
  L.~Xiao, D.M.~York D.M., and P.A. Kollman.
\newblock {Amber} 2018.
\newblock \url{http://ambermd.org}, 2018.

\bibitem{Longuet-Higgins1963}
Hugh~C. Longuet-Higgins.
\newblock The symmetry groups of non-rigid molecules.
\newblock {\em Mol. Phys.}, 6(5):445--460, 1963.

\bibitem{tuckerman2002ab}
Mark~E. Tuckerman.
\newblock Ab initio molecular dynamics: {B}asic concepts, current trends and
  novel applications.
\newblock {\em J. Phys. Condens. Matter}, 14(50):R1297, 2002.

\bibitem{rupp2012fast}
Matthias Rupp, Alexandre Tkatchenko, Klaus-Robert M{\"u}ller, and O.~Anatole
  Von~Lilienfeld.
\newblock Fast and accurate modeling of molecular atomization energies with
  machine learning.
\newblock {\em Phys. Rev. Lett.}, 108(5):58301, 2012.

\bibitem{Hansen2013}
Katja Hansen, Gr{\'{e}}goire Montavon, Franziska Biegler, Siamac Fazli,
  Matthias Rupp, Matthias Scheffler, O.~Anatole von Lilienfeld, Alexandre
  Tkatchenko, and Klaus-Robert M{\"{u}}ller.
\newblock Assessment and validation of machine learning methods for predicting
  molecular atomization energies.
\newblock {\em J. Chem. Theory Comput.}, 9(8):3404--3419, 2013.

\bibitem{Hansen2015}
Katja Hansen, Franziska Biegler, Raghunathan Ramakrishnan, Wiktor Pronobis,
  O~Anatole von Lilienfeld, Klaus-Robert M{\"{u}}ller, and Alexandre
  Tkatchenko.
\newblock Machine learning predictions of molecular properties: {A}ccurate
  many-body potentials and nonlocality in chemical space.
\newblock {\em J. Phys. Chem. Lett.}, 6(12):2326--2331, 2015.

\bibitem{Rupp2015}
Matthias Rupp, Raghunathan Ramakrishnan, and O.~Anatole von Lilienfeld.
\newblock Machine learning for quantum mechanical properties of atoms in
  molecules.
\newblock {\em J. Phys. Chem. Lett.}, 6(16):3309--3313, 2015.

\bibitem{botu2015adaptive}
Venkatesh Botu and Rampi Ramprasad.
\newblock Adaptive machine learning framework to accelerate ab initio molecular
  dynamics.
\newblock {\em Int. J. Quantum Chem.}, 115(16):1074--1083, 2015.

\bibitem{Hirn2015}
Matthew Hirn, Nicolas Poilvert, and St{\'{e}}phane Mallat.
\newblock Quantum energy regression using scattering transforms.
\newblock {\em CoRR}, abs/1502.02077, 2015.

\bibitem{deltaML2015}
Raghunathan Ramakrishnan, Pavlo~O. Dral, Matthias Rupp, and O.~Anatole von
  Lilienfeld.
\newblock Big data meets quantum chemistry approximations: {T}he
  $\delta$-machine learning approach.
\newblock {\em J. Chem. Theory Comput.}, 11(5):2087--2096, 2015.

\bibitem{Ceriotti2016}
Sandip De, Albert~P Bart{\'o}k, G{\'a}bor Cs{\'a}nyi, and Michele Ceriotti.
\newblock Comparing molecules and solids across structural and alchemical
  space.
\newblock {\em Phys. Chem. Chem. Phys.}, 18(20):13754--13769, 2016.

\bibitem{artrith2017efficient}
Nongnuch Artrith, Alexander Urban, and Gerbrand Ceder.
\newblock Efficient and accurate machine-learning interpolation of atomic
  energies in compositions with many species.
\newblock {\em Phys. Rev. B}, 96(1):14112, 2017.

\bibitem{Ceriotti2017}
Albert~P. Bart{\'o}k, Sandip De, Carl Poelking, Noam Bernstein, James~R.
  Kermode, G{\'a}bor Cs{\'a}nyi, and Michele Ceriotti.
\newblock Machine learning unifies the modeling of materials and molecules.
\newblock {\em Sci. Adv.}, 3(12):e1701816, 2017.

\bibitem{Glielmo2017}
Aldo Glielmo, Peter Sollich, and Alessandro De~Vita.
\newblock Accurate interatomic force fields via machine learning with covariant
  kernels.
\newblock {\em Phys. Rev. B}, 95:214302, 2017.

\bibitem{yao2017many}
Kun Yao, John~E. Herr, and John Parkhill.
\newblock The many-body expansion combined with neural networks.
\newblock {\em J. Chem. Phys.}, 146(1):14106, 2017.

\bibitem{john2017many}
ST~John and G{\'{a}}bor Cs{\'{a}}nyi.
\newblock Many-body coarse-grained interactions using {G}aussian approximation
  potentials.
\newblock {\em J. Phys. Chem. B}, 121(48):10934--10949, 2017.

\bibitem{faber2017prediction}
Felix~A. Faber, Luke Hutchison, Bing Huang, Justin Gilmer, Samuel~S.
  Schoenholz, George~E. Dahl, Oriol Vinyals, Steven Kearnes, Patrick~F. Riley,
  and O.~Anatole von Lilienfeld.
\newblock Prediction errors of molecular machine learning models lower than
  hybrid {DFT} error.
\newblock {\em J. Chem. Theory Comput.}, 13(11):5255--5264, 2017.

\bibitem{eickenberg2018solid}
Michael Eickenberg, Georgios Exarchakis, Matthew Hirn, St{\'e}phane Mallat, and
  Louis Thiry.
\newblock Solid harmonic wavelet scattering for predictions of molecule
  properties.
\newblock {\em J. Chem. Phys.}, 148(24):241732, 2018.

\bibitem{glielmo2018efficient}
Aldo Glielmo, Claudio Zeni, and Alessandro De~Vita.
\newblock Efficient nonparametric n-body force fields from machine learning.
\newblock {\em Phys. Rev. B}, 97(18):184307, 2018.

\bibitem{tang2018atomistic}
Yu-Hang Tang, Dongkun Zhang, and George~Em Karniadakis.
\newblock An atomistic fingerprint algorithm for learning ab initio molecular
  force fields.
\newblock {\em J. Chem. Phys.}, 148(3):34101, 2018.

\bibitem{Grisafi2018}
Andrea Grisafi, David~M. Wilkins, G\'abor Cs\'anyi, and Michele Ceriotti.
\newblock Symmetry-adapted machine learning for tensorial properties of
  atomistic systems.
\newblock {\em Phys. Rev. Lett.}, 120:36002, 2018.

\bibitem{pronobis2018many}
Wiktor Pronobis, Alexandre Tkatchenko, and Klaus-Robert M{\"u}ller.
\newblock Many-body descriptors for predicting molecular properties with
  machine learning: Analysis of pairwise and three-body interactions in
  molecules.
\newblock {\em J. Chem. Theory Comput.}, 14(6):2991--3003, 2018.

\bibitem{Behler2007}
J{\"{o}}rg Behler and Michele Parrinello.
\newblock {Generalized neural-network representation of high-dimensional
  potential-energy surfaces}.
\newblock {\em Phys. Rev. Lett.}, 98(14):146401, 2007.

\bibitem{Bartok2010}
Albert~P. Bart{\'{o}}k, Mike~C. Payne, Risi Kondor, and G{\'{a}}bor
  Cs{\'{a}}nyi.
\newblock {G}aussian approximation potentials: {T}he accuracy of quantum
  mechanics, without the electrons.
\newblock {\em Phys. Rev. Lett.}, 104(13):136403, 2010.

\bibitem{Behler2012}
K.~V.~Jovan Jose, Nongnuch Artrith, and J{\"{o}}rg Behler.
\newblock Construction of high-dimensional neural network potentials using
  environment-dependent atom pairs.
\newblock {\em J. Chem. Phys.}, 136(19):194111, 2012.

\bibitem{Bartok2013}
Albert~P. Bart{\'{o}}k, Risi Kondor, and G{\'{a}}bor Cs{\'{a}}nyi.
\newblock {On representing chemical environments}.
\newblock {\em Phys. Rev. B}, 87(18):184115, 2013.

\bibitem{Montavon2013a}
Gr{\'{e}}goire Montavon, Matthias Rupp, Vivekanand Gobre, Alvaro
  Vazquez-Mayagoitia, Katja Hansen, Alexandre Tkatchenko, Klaus-Robert
  M{\"{u}}ller, and O.~Anatole von Lilienfeld.
\newblock Machine learning of molecular electronic properties in chemical
  compound space.
\newblock {\em New J. Phys.}, 15(9):95003, 2013.

\bibitem{Bartok2015}
Albert~P. Bart{\'{o}}k and G{\'{a}}bor Cs{\'{a}}nyi.
\newblock {G}aussian approximation potentials: {A} brief tutorial introduction.
\newblock {\em Int. J. Quantum Chem.}, 115(16):1051--1057, 2015.

\bibitem{Ramprasad2015}
V.~Botu and R.~Ramprasad.
\newblock Learning scheme to predict atomic forces and accelerate materials
  simulations.
\newblock {\em Phys. Rev. B}, 92:94306, 2015.

\bibitem{Tristan2015}
Tristan Bereau, Denis Andrienko, and O.~Anatole von Lilienfeld.
\newblock Transferable atomic multipole machine learning models for small
  organic molecules.
\newblock {\em J. Chem. Theory Comput.}, 11(7):3225--3233, 2015.

\bibitem{DeVita2015}
Zhenwei Li, James~R. Kermode, and Alessandro De~Vita.
\newblock Molecular dynamics with on-the-fly machine learning of
  quantum-mechanical forces.
\newblock {\em Phys. Rev. Lett.}, 114:96405, 2015.

\bibitem{Behler2016}
J{\"{o}}rg Behler.
\newblock Perspective: {M}achine learning potentials for atomistic simulations.
\newblock {\em J. Chem. Phys.}, 145(17):170901, 2016.

\bibitem{Brockherde2017}
Felix Brockherde, Leslie Vogt, Li~Li, Mark~E. Tuckerman, Kieron Burke, and
  Klaus-Robert M{\"u}ller.
\newblock Bypassing the {Kohn-Sham} equations with machine learning.
\newblock {\em Nat. Commun.}, 8:872, 2017.

\bibitem{Gastegger2017}
Michael Gastegger, Jorg Behler, and Philipp Marquetand.
\newblock Machine learning molecular dynamics for the simulation of infrared
  spectra.
\newblock {\em Chem. Sci.}, 8:6924--6935, 2017.

\bibitem{Schutt2017}
Kristof~T. Sch{\"u}tt, Farhad Arbabzadah, Stefan Chmiela, Klaus-Robert
  M{\"u}ller, and Alexandre Tkatchenko.
\newblock Quantum-chemical insights from deep tensor neural networks.
\newblock {\em Nat. Commun.}, 8:13890, 2017.

\bibitem{schutt2017schnet}
Kristof Sch{\"u}tt, Pieter-Jan Kindermans, Huziel~E. Sauceda, Stefan Chmiela,
  Alexandre Tkatchenko, and Klaus-Robert M{\"u}ller.
\newblock {SchNet}: {A} continuous-filter convolutional neural network for
  modeling quantum interactions.
\newblock In {\em Adv. Neural. Inf. Process. Syst. 31}, pages 991--1001, 2017.

\bibitem{SchNet2018}
Kristof~T. Sch\"utt, H.~E. Sauceda, Pieter-Jan Kindermans, Alexandre
  Tkatchenko, and Klaus-Robert M\"uller.
\newblock {SchNet} -- {A} deep learning architecture for molecules and
  materials.
\newblock {\em J. Chem. Phys.}, 148(24):241722, 2018.

\bibitem{huang1707dna}
Bing Huang and O.~Anatole von Lilienfeld.
\newblock The {"DNA"} of chemistry: {S}calable quantum machine learning with
  "amons".
\newblock {\em arXiv preprint arXiv:1707.04146}, 2017.

\bibitem{huan2017universal}
Tran~Doan Huan, Rohit Batra, James Chapman, Sridevi Krishnan, Lihua Chen, and
  Rampi Ramprasad.
\newblock A universal strategy for the creation of machine learning-based
  atomistic force fields.
\newblock {\em {NPJ} Comput. Mater.}, 3(1):37, 2017.

\bibitem{Shapeev2017}
Evgeny~V. Podryabinkin and Alexander~V. Shapeev.
\newblock Active learning of linearly parametrized interatomic potentials.
\newblock {\em Comput. Mater. Sci.}, 140:171--180, 2017.

\bibitem{dral2017structure}
Pavlo~O. Dral, Alec Owens, Sergei~N. Yurchenko, and Walter Thiel.
\newblock Structure-based sampling and self-correcting machine learning for
  accurate calculations of potential energy surfaces and vibrational levels.
\newblock {\em J. Chem. Phys.}, 146(24):244108, 2017.

\bibitem{zhang2018deep}
Linfeng Zhang, Jiequn Han, Han Wang, Roberto Car, and E.~Weinan.
\newblock Deep potential molecular dynamics: {A} scalable model with the
  accuracy of quantum mechanics.
\newblock {\em Phys. Rev. Lett.}, 120(14):143001, 2018.

\bibitem{lubbers2018hierarchical}
Nicholas Lubbers, Justin~S. Smith, and Kipton Barros.
\newblock Hierarchical modeling of molecular energies using a deep neural
  network.
\newblock {\em J. Chem. Phys.}, 148(24):241715, 2018.

\bibitem{ryczko2018convolutional}
Kevin Ryczko, Kyle Mills, Iryna Luchak, Christa Homenick, and Isaac Tamblyn.
\newblock Convolutional neural networks for atomistic systems.
\newblock {\em Comput. Mater. Sci.}, 149:134--142, 2018.

\bibitem{kanamori2018exploring}
Kenta Kanamori, Kazuaki Toyoura, Junya Honda, Kazuki Hattori, Atsuto Seko,
  Masayuki Karasuyama, Kazuki Shitara, Motoki Shiga, Akihide Kuwabara, and
  Ichiro Takeuchi.
\newblock Exploring a potential energy surface by machine learning for
  characterizing atomic transport.
\newblock {\em Phys. Rev. B}, 97(12):125124, 2018.

\bibitem{hy2018predicting}
Truong~Son Hy, Shubhendu Trivedi, Horace Pan, Brandon~M. Anderson, and Risi
  Kondor.
\newblock Predicting molecular properties with covariant compositional
  networks.
\newblock {\em J. Chem. Phys.}, 148(24):241745, 2018.

\bibitem{Clementi2018}
Jiang Wang, Christoph Wehmeyer, Frank No{\'e}, and Cecilia Clementi.
\newblock Machine learning of coarse-grained molecular dynamics force fields,
  2018.

\bibitem{Tristan}
Tristan Bereau, Robert~A. DiStasio~Jr, Alexandre Tkatchenko, and O~Anatole
  Von~Lilienfeld.
\newblock Non-covalent interactions across organic and biological subsets of
  chemical space: {P}hysics-based potentials parametrized from machine
  learning.
\newblock {\em J. Chem. Phys.}, 148(24):241706, 2018.

\bibitem{noe2018}
Andreas Mardt, Luca Pasquali, Hao Wu, and Frank No{\'e}.
\newblock {VAMPnets} for deep learning of molecular kinetics.
\newblock {\em Nat. Commun.}, 9(1):5, 2018.

\bibitem{noe2018b}
Frank No{\'e} and Hao Wu.
\newblock Boltzmann generators -- {S}ampling equilibrium states of many-body
  systems with deep learning.
\newblock {\em arXiv preprint arXiv:1812.01729}, 2018.

\bibitem{thomas2018tensor}
Nathaniel Thomas, Tess Smidt, Steven Kearnes, Lusann Yang, Li~Li, Kai Kohlhoff,
  and Patrick Riley.
\newblock Tensor field networks: {R}otation-and translation-equivariant neural
  networks for {3D} point clouds.
\newblock {\em arXiv preprint arXiv:1802.08219}, 2018.

\bibitem{smith2018less}
Justin~S. Smith, Ben Nebgen, Nicholas Lubbers, Olexandr Isayev, and Adrian
  Roitberg.
\newblock Less is more: {S}ampling chemical space with active learning.
\newblock {\em J. Chem. Phys.}, 148(24):241733, 2018.

\bibitem{gubaev2018machine}
Konstantin Gubaev, Evgeny~V. Podryabinkin, and Alexander~V. Shapeev.
\newblock Machine learning of molecular properties: {L}ocality and active
  learning.
\newblock {\em J. Chem. Phys.}, 148(24):241727, 2018.

\bibitem{FCHL2018}
Felix~A. Faber, Anders~S. Christensen, Bing Huang, and O.~Anatole von
  Lilienfeld.
\newblock Alchemical and structural distribution based representation for
  universal quantum machine learning.
\newblock {\em J. Chem. Phys.}, 148(24):241717, 2018.

\bibitem{christensen2019operators}
Anders~S. Christensen, Felix~A. Faber, and O.~Anatole von Lilienfeld.
\newblock Operators in quantum machine learning: {R}esponse properties in
  chemical space.
\newblock {\em J. Phys. Chem.}, 150(6):64105, 2019.

\bibitem{winter2019}
Robin Winter, Floriane Montanari, Frank No{\'e}, and Djork-Arn{\'e} Clevert.
\newblock Learning continuous and data-driven molecular descriptors by
  translating equivalent chemical representations.
\newblock {\em Chem. Sci.}, 2019.

\bibitem{gubaev2019accelerating}
Konstantin Gubaev, Evgeny~V. Podryabinkin, Gus L.~W. Hart, and Alexander~V.
  Shapeev.
\newblock Accelerating high-throughput searches for new alloys with active
  learning of interatomic potentials.
\newblock {\em Comput. Mater. Sci.}, 156:148--156, 2019.

\bibitem{marx1996ab}
Dominik Marx and Michele Parrinello.
\newblock Ab initio path integral molecular dynamics: {B}asic ideas.
\newblock {\em J. Chem. Phys.}, 104(11):4077--4082, 1996.

\bibitem{szabo2012modern}
Attila Szabo and Neil~S. Ostlund.
\newblock {\em Modern quantum chemistry: {I}ntroduction to advanced electronic
  structure theory}.
\newblock Courier Corporation, 2012.

\bibitem{marx2009ab}
Dominik Marx and J{\"u}rg Hutter.
\newblock {\em Ab initio molecular dynamics: {B}asic theory and advanced
  methods}.
\newblock Cambridge University Press, 2009.

\bibitem{markland2018nuclear}
Thomas~E. Markland and Michele Ceriotti.
\newblock Nuclear quantum effects enter the mainstream.
\newblock {\em Nat. Rev. Chem.}, 2:109, 2018.

\bibitem{tuckerman2010statistical}
Mark Tuckerman.
\newblock {\em Statistical mechanics: {T}heory and molecular simulation}.
\newblock Oxford University Press, 2010.

\bibitem{stone2013theory}
Anthony Stone.
\newblock {\em The theory of intermolecular forces}.
\newblock Oxford University Press, 2013.

\bibitem{patkowski2005accurate}
Konrad Patkowski, Garold Murdachaew, Cheng-Ming Fou, and Krzysztof Szalewicz.
\newblock Accurate ab initio potential for argon dimer including highly
  repulsive region.
\newblock {\em Molecular Physics}, 103(15-16):2031--2045, 2005.

\bibitem{hohenberg1964inhomogeneous}
Pierre Hohenberg and Walter Kohn.
\newblock Inhomogeneous electron gas.
\newblock {\em Phys. Rev.}, 136(3b):B864, 1964.

\bibitem{kohn1965self}
Walter Kohn and Lu~Jeu Sham.
\newblock Self-consistent equations including exchange and correlation effects.
\newblock {\em Phys. Rev.}, 140(4a):A1133, 1965.

\bibitem{tuckerman2000understanding}
Mark~E. Tuckerman and Glenn~J. Martyna.
\newblock Understanding modern molecular dynamics: {T}echniques and
  applications, 2000.

\bibitem{pereyaslavets2018importance}
Leonid Pereyaslavets, Igor Kurnikov, Ganesh Kamath, Oleg Butin, Alexey
  Illarionov, Igor Leontyev, Michael Olevanov, Michael Levitt, Roger~D.
  Kornberg, and Boris Fain.
\newblock On the importance of accounting for nuclear quantum effects in ab
  initio calibrated force fields in biological simulations.
\newblock {\em Proc. Natl. Acad. Sci. U.S.A.}, 115(36):8878--8882, 2018.

\bibitem{lamaire2019importance}
Aran Lamaire, Jelle Wieme, Sven M.~J. Rogge, Michel Waroquier, and Veronique
  Van~Speybroeck.
\newblock On the importance of anharmonicities and nuclear quantum effects in
  modelling the structural properties and thermal expansion of {MOF-5}.
\newblock {\em J. Chem. Phys.}, 150(9):94503, 2019.

\bibitem{tuckerman1993efficient}
Mark~E. Tuckerman, Bruce~J. Berne, Glenn~J. Martyna, and Michael~L. Klein.
\newblock Efficient molecular dynamics and hybrid monte carlo algorithms for
  path integrals.
\newblock {\em J. Chem. Phys.}, 99(4):2796--2808, 1993.

\bibitem{balog2000constant}
E.~Balog, A.~L. Hughes, and Glenn~J. Martyna.
\newblock Constant pressure path integral molecular dynamics studies of quantum
  effects in the liquid state properties of n-alkanes.
\newblock {\em J. Chem. Phys.}, 112(2):870--880, 2000.

\bibitem{martyna1999molecular}
Glenn~J. Martyna, Adam Hughes, and Mark~E. Tuckerman.
\newblock Molecular dynamics algorithms for path integrals at constant
  pressure.
\newblock {\em J. Chem. Phys.}, 110(7):3275--3290, 1999.

\bibitem{chandler1981exploiting}
David Chandler and Peter~G. Wolynes.
\newblock Exploiting the isomorphism between quantum theory and classical
  statistical mechanics of polyatomic fluids.
\newblock {\em J. Chem. Phys.}, 74(7):4078--4095, 1981.

\bibitem{noether1918invarianten}
Emmy Noether.
\newblock Invarianten beliebiger {D}ifferentialausdr{\"u}cke.
\newblock {\em G{\"o}tt. Nachr., mathematisch-physikalische Klasse},
  1918:37--44, 1918.

\bibitem{scholkopf2001learning}
Bernhard Sch{\"o}lkopf and Alexander~J. Smola.
\newblock {\em Learning with kernels: {S}upport vector machines,
  regularization, optimization, and beyond}.
\newblock MIT Press, 2001.

\bibitem{wahba1990spline}
Grace Wahba.
\newblock {\em Spline models for observational data}, volume~59.
\newblock SIAM, 1990.

\bibitem{scholkopf2001generalized}
Bernhard Sch{\"o}lkopf, Ralf Herbrich, and Alex~J. Smola.
\newblock A generalized representer theorem.
\newblock In {\em International conference on computational learning theory},
  pages 416--426. Springer, 2001.

\bibitem{Muller2001}
Klaus-Robert M{\"{u}}ller, Sebastian Mika, Gunnar R{\"{a}}tsch, Koji Tsuda, and
  Bernhard Sch{\"{o}}lkopf.
\newblock An introduction to kernel-based learning algorithms.
\newblock {\em IEEE Trans. Neural Netw. Learn. Syst.}, 12(2):181--201, 2001.

\bibitem{rasmussen2004gaussian}
Carl~E. Rasmussen.
\newblock Gaussian processes in machine learning.
\newblock In {\em Advanced lectures on machine learning}, pages 63--71.
  Springer, 2004.

\bibitem{duvenaud2014automatic}
David Duvenaud.
\newblock {\em Automatic model construction with {G}aussian processes}.
\newblock PhD thesis, University of Cambridge, 2014.

\bibitem{micchelli2006universal}
Charles~A. Micchelli, Yuesheng Xu, and Haizhang Zhang.
\newblock Universal kernels.
\newblock {\em J. Mach. Learn. Res.}, 7(Dec):2651--2667, 2006.

\bibitem{damianou2013deep}
Andreas Damianou and Neil Lawrence.
\newblock Deep {G}aussian processes.
\newblock In {\em Artificial Intelligence and Statistics}, pages 207--215,
  2013.

\bibitem{Lanczos1949}
Cornelius Lanczos.
\newblock {\em The variational principles of mechanics}.
\newblock University of Toronto Press, 1949.

\bibitem{brading2003symmetries}
Katherine Brading and Elena Castellani.
\newblock {\em Symmetries in physics: {P}hilosophical reflections}.
\newblock Cambridge University Press, 2003.

\bibitem{narcowich1994generalized}
Francis~J. Narcowich and Joseph~D Ward.
\newblock Generalized {H}ermite interpolation via matrix-valued conditionally
  positive definite functions.
\newblock {\em Math. Comput.}, 63(208):661--687, 1994.

\bibitem{solak2003derivative}
Ercan Solak, Roderick Murray-Smith, William~E Leithead, Douglas~J. Leith, and
  Carl~E. Rasmussen.
\newblock Derivative observations in {G}aussian process models of dynamic
  systems.
\newblock In {\em Adv. Neural. Inf. Process. Syst.}, pages 1057--1064, 2003.

\bibitem{donoho2006compressed}
David~L Donoho.
\newblock Compressed sensing.
\newblock {\em IEEE Trans. Inf. Theory}, 52(4):1289--1306, 2006.

\bibitem{yu2014learning}
Felix~X Yu, Krzysztof Choromanski, Sanjiv Kumar, Tony Jebara, and Shih-Fu
  Chang.
\newblock On learning from label proportions.
\newblock {\em arXiv preprint arXiv:1402.5902}, 2014.

\bibitem{mackay1998introduction}
David J.~C. MacKay.
\newblock {\em Introduction to {G}aussian processes}, volume 168 of {\em NATO
  ASI Series F: Computer and Systems Sciences}.
\newblock Springer, 1998.

\bibitem{smola1998connection}
Alex~J Smola, Bernhard Sch{\"o}lkopf, and Klaus-Robert M{\"u}ller.
\newblock The connection between regularization operators and support vector
  kernels.
\newblock {\em Neural networks}, 11(4):637--649, 1998.

\bibitem{heil2018metrics}
Christopher Heil.
\newblock {\em Metrics, Norms, Inner Products, and Operator Theory}.
\newblock Birkh\"auser Basel, 2018.

\bibitem{rahimi2008random}
Ali Rahimi and Benjamin Recht.
\newblock Random features for large-scale kernel machines.
\newblock In {\em Adv. Neural. Inf. Process. Syst.}, pages 1177--1184, 2008.

\bibitem{politzer2018hellmann}
Peter Politzer and Jane~S. Murray.
\newblock The {H}ellmann-{F}eynman theorem: {A} perspective.
\newblock {\em J. Mol. Model.}, 24(9):266, 2018.

\bibitem{feynman1939forces}
Richard~Phillips Feynman.
\newblock Forces in molecules.
\newblock {\em Phys. Rev.}, 56(4):340, 1939.

\bibitem{Shannon1998}
C.E. Shannon.
\newblock {Communication in the Presence of Noise}.
\newblock {\em Proceedings of the IEEE}, 86(2):447--457, 1998.

\bibitem{Snyder2012}
John~C Snyder, Matthias Rupp, Katja Hansen, Klaus-Robert M{\"u}ller, and Kieron
  Burke.
\newblock Finding density functionals with machine learning.
\newblock {\em Phys. Rev. Lett.}, 108(25):253002, 2012.

\bibitem{Snyder2015}
John~C Snyder, Matthias Rupp, Klaus-Robert M{\"u}ller, and Kieron Burke.
\newblock Nonlinear gradient denoising: {F}inding accurate extrema from
  inaccurate functional derivatives.
\newblock {\em Int. J. Quantum Chem.}, 115(16):1102--1114, 2015.

\bibitem{Scholkopf1998}
Bernhard Sch{\"o}lkopf, Alexander Smola, and Klaus-Robert M{\"u}ller.
\newblock Nonlinear component analysis as a kernel eigenvalue problem.
\newblock {\em Neural Comput.}, 10(5):1299--1319, 1998.

\bibitem{Scholkopf1999}
Bernhard Sch{\"o}lkopf, Sebastian Mika, Chris J.~C. Burges, Philipp Knirsch,
  Klaus-Robert M{\"u}ller, Gunnar R{\"a}tsch, and Alexander~J. Smola.
\newblock Input space versus feature space in kernel-based methods.
\newblock {\em IEEE Transactions on Neural Networks}, 10(5):1000--1017, 1999.

\bibitem{micchelli2005learning}
Charles~A. Micchelli and Massimiliano Pontil.
\newblock On learning vector-valued functions.
\newblock {\em Neural Comput.}, 17(1):177--204, 2005.

\bibitem{Caponnetto2008}
Andrea Caponnetto, Charles~A. Micchelli, Massimiliano Pontil, and Yiming Ying.
\newblock Universal multi-task kernels.
\newblock {\em J. Mach. Learn. Res.}, 9:1615--1646, 2008.

\bibitem{Sindhwani1964}
Vikas Sindhwani, H{\`{a}}~Quang Minh, and Aur{\'e}lie~C. Lozano.
\newblock Scalable matrix-valued kernel learning for high-dimensional nonlinear
  multivariate regression and granger causality.
\newblock In {\em Proc. 29th Conference on Uncertainty in Artificial
  Intelligence}, Uai'13, pages 586--595, Arlington, Virginia, United States,
  2013. AUAI Press.

\bibitem{friedman2001elements}
Trevor Hastie, Robert Tibshirani, and Jerome~H. Friedman.
\newblock {\em The elements of statistical learning: {D}ata mining, inference,
  and prediction}.
\newblock Springer series in statistics. Springer, 2009.

\bibitem{alvarez2012kernels}
Mauricio~A. Alvarez, Lorenzo Rosasco, Neil~D. Lawrence, et~al.
\newblock Kernels for vector-valued functions: {A} review.
\newblock {\em Foundations and Trends in Machine Learning}, 4(3):195--266,
  2012.

\bibitem{boyle2005dependent}
Phillip Boyle and Marcus Frean.
\newblock Dependent {G}aussian processes.
\newblock In {\em Adv. Neural. Inf. Process. Syst.}, pages 217--224, 2005.

\bibitem{micchelli2005kernels}
Charles~A. Micchelli and Massimiliano Pontil.
\newblock Kernels for multi-task learning.
\newblock In {\em Adv. Neural. Inf. Process. Syst.}, pages 921--928, 2005.

\bibitem{baldassarre2012multi}
Luca Baldassarre, Lorenzo Rosasco, Annalisa Barla, and Alessandro Verri.
\newblock Multi-output learning via spectral filtering.
\newblock {\em Machine learning}, 87(3):259--301, 2012.

\bibitem{graepel2003solving}
Thore Graepel.
\newblock Solving noisy linear operator equations by {G}aussian processes:
  {A}pplication to ordinary and partial differential equations.
\newblock In {\em International Conference on Machine Learning}, pages
  234--241, 2003.

\bibitem{sarkka2011linear}
Simo S{\"a}rkk{\"a}.
\newblock Linear operators and stochastic partial differential equations in
  {G}aussian process regression.
\newblock In {\em International Conference on Artificial Neural Networks},
  pages 151--158. Springer, 2011.

\bibitem{constantinescu2013physics}
Emil~M. Constantinescu and Mihai Anitescu.
\newblock Physics-based covariance models for {G}aussian processes with
  multiple outputs.
\newblock {\em International Journal for Uncertainty Quantification}, 3(1),
  2013.

\bibitem{nguyen2015gaussian}
Ngoc~Cuong Nguyen and Jaime Peraire.
\newblock Gaussian functional regression for linear partial differential
  equations.
\newblock {\em Comput. Methods Appl. Mech. Eng.}, 287:69--89, 2015.

\bibitem{jidling2017linearly}
Carl Jidling, Niklas Wahlstr{\"o}m, Adrian Wills, and Thomas~B Sch{\"o}n.
\newblock Linearly constrained {G}aussian processes.
\newblock In {\em Adv. Neural. Inf. Process. Syst.}, pages 1215--1224, 2017.

\bibitem{Helmholz1858}
Hermann Helmholz.
\newblock {\"{U}}ber {I}ntegrale der hydrodynamischen {G}leichungen, welche den
  {W}irbelbewegungen entsprechen.
\newblock {\em Journal f{\"{u}}r die reine und angewandte {M}athematik},
  55:25--55, 1858.

\bibitem{matern1986spatial}
Bertil Mat{\'{e}}rn.
\newblock {\em Spatial Variation}.
\newblock Lecture notes in statistics. Springer, 1986.

\bibitem{stein1999}
Michael~L. Stein.
\newblock {\em Interpolation of Spatial Data - Some Theory for Kriging}.
\newblock Springer New York, 1999.

\bibitem{Gradshteyn2007}
I.~S. Gradshteyn and I.~M. Ryzhik.
\newblock {\em Table of Integrals, Series, and Products, ({E}quation 8.468)}.
\newblock 7 edition, 2007.

\bibitem{Gneiting2010}
Tilmann Gneiting, William Kleiber, and Martin Schlather.
\newblock Mat{\'{e}}rn cross-covariance functions for multivariate random
  fields.
\newblock {\em J. Am. Stat. Assoc.}, 105(491):1167--1177, 2010.

\bibitem{rapaport2004art}
Dennis~C. Rapaport and Dennis C.~Rapaport Rapaport.
\newblock {\em The art of molecular dynamics simulation}.
\newblock Cambridge University Press, 2004.

\bibitem{PBE1996}
John~P. Perdew, Kieron Burke, and Matthias Ernzerhof.
\newblock Generalized gradient approximation made simple.
\newblock {\em Phys. Rev. Lett.}, 77:3865--3868, 1996.

\bibitem{TS}
Alexandre Tkatchenko and Matthias Scheffler.
\newblock Accurate molecular van der waals interactions from ground-state
  electron density and free-atom reference data.
\newblock {\em Phys. Rev. Lett.}, 102(7):73005, 2009.

\bibitem{ceriotti2014pi}
Michele Ceriotti, Joshua More, and David~E. Manolopoulos.
\newblock {i-PI}: {A} python interface for ab initio path integral molecular
  dynamics simulations.
\newblock {\em Comput. Phys. Commun.}, 185(3):1019--1026, 2014.

\bibitem{chmiela2019}
Stefan Chmiela, Huziel~E. Sauceda, Igor Poltavsky, Klaus-Robert M\"{u}ller, and
  Alexandre Tkatchenko.
\newblock {sGDML}: {C}onstructing accurate and data efficient molecular force
  fields using machine learning.
\newblock {\em Comput. Phys. Commun.}, 2019.

\bibitem{reilly2015van}
Anthony~M. Reilly and Alexandre Tkatchenko.
\newblock van der {W}aals dispersion interactions in molecular materials:
  {B}eyond pairwise additivity.
\newblock {\em Chem. Sci.}, 6(6):3289--3301, 2015.

\bibitem{Sauceda2019}
Huziel~E. Sauceda, Stefan Chmiela, Igor Poltavsky, Klaus-Robert M\"{u}ller, and
  Alexandre Tkatchenko.
\newblock Molecular force fields with gradient-domain machine learning:
  Construction and application to dynamics of small molecules with coupled
  cluster forces.
\newblock {\em J. Chem. Phys}, 150(11):114102, 2019.

\bibitem{osborne2010bayesian}
Michael~A Osborne.
\newblock {\em Bayesian {G}aussian processes for sequential prediction,
  optimisation and quadrature}.
\newblock PhD thesis, University of Oxford, 2010.

\bibitem{osborne2009gaussian}
Michael~A. Osborne, Roman Garnett, and Stephen~J. Roberts.
\newblock Gaussian processes for global optimization.
\newblock In {\em 3rd international conference on learning and intelligent
  optimization}, 2009.

\bibitem{ase17}
Ask~Hjorth Larsen, Jens~J{\o}rgen Mortensen, Jakob Blomqvist, Ivano~E Castelli,
  Rune Christensen, Marcin Du{\l}ak, Jesper Friis, Michael~N Groves, Bj{\o}rk
  Hammer, Cory Hargus, et~al.
\newblock The atomic simulation environment -- {A} python library for working
  with atoms.
\newblock {\em J. Phys. Condens. Matter}, 29(27):273002, 2017.

\bibitem{ipiv2}
Venkat Kapil, Mariana Rossi, Ondrej Marsalek, Riccardo Petraglia, Yair Litman,
  Thomas Spura, Bingqing Cheng, Alice Cuzzocrea, Robert~H Mei{\ss}ner, David~M
  Wilkins, et~al.
\newblock {i-PI} 2.0: {A} universal force engine for advanced molecular
  simulations.
\newblock {\em Comput. Phys. Commun.}, 236:214--223, 2019.

\bibitem{wilson1955molecular}
Edgar~B. Wilson.
\newblock {\em Molecular Vibrations: {T}he Theory of Infrared and Raman
  Vibrational Spectra}.
\newblock McGraw-Hill Interamericana, 1955.

\bibitem{pachauri2013solving}
Deepti Pachauri, Risi Kondor, and Vikas Singh.
\newblock Solving the multi-way matching problem by permutation
  synchronization.
\newblock In {\em Adv. Neural. Inf. Process. Syst.}, pages 1860--1868, 2013.

\bibitem{Schiavinato2015}
Michele Schiavinato, Andrea Gasparetto, and Andrea Torsello.
\newblock {\em Transitive Assignment Kernels for Structural Classification},
  pages 146--159.
\newblock Springer International Publishing, Cham, 2015.

\bibitem{Kriege2016}
Nils~M. Kriege, Pierre-Louis Giscard, and Richard~C. Wilson.
\newblock On valid optimal assignment kernels and applications to graph
  classification.
\newblock In {\em Adv. Neural. Inf. Process. Syst. 30}, pages 1623--1631, 2016.

\bibitem{Vert2008}
Jean{-}Philippe Vert.
\newblock The optimal assignment kernel is not positive definite.
\newblock {\em CoRR}, abs/0801.4061, 2008.

\bibitem{Umeyama1988}
Shinji Umeyama.
\newblock An eigendecomposition approach to weighted graph matching problems.
\newblock {\em IEEE Trans. Pattern Anal. Mach. Intell.}, 10(5):695--703, 1988.

\bibitem{Kuhn1955}
Harold~William Kuhn.
\newblock The {H}ungarian method for the assignment problem.
\newblock {\em Nav. Res. Logist.}, 2(1-2):83--97, 1955.

\bibitem{karvonen2018fully}
Toni Karvonen and Simo S\"arkk\"a.
\newblock Fully symmetric kernel quadrature.
\newblock {\em SIAM Journal on Scientific Computing}, 40(2):A697--a720, 2018.

\bibitem{haasdonk2007invariant}
Bernard Haasdonk and Hans Burkhardt.
\newblock Invariant kernel functions for pattern analysis and machine learning.
\newblock {\em Machine learning}, 68(1):35--61, 2007.

\bibitem{FHIaims2009}
Volker Blum, Ralf Gehrke, Felix Hanke, Paula Havu, Ville Havu, Xinguo Ren,
  Karsten Reuter, and Matthias Scheffler.
\newblock Ab initio molecular simulations with numeric atom-centered orbitals.
\newblock {\em Comput. Phys. Commun.}, 180(11):2175--2196, 2009.

\bibitem{psi42012}
Justin~M. Turney, Andrew~C. Simmonett, Robert~M. Parrish, Edward~G. Hohenstein,
  Francesco~A. Evangelista, Justin~T. Fermann, Benjamin~J. Mintz, Lori~A.
  Burns, Jeremiah~J. Wilke, Micah~L. Abrams, Nicholas~J. Russ, Matthew~L.
  Leininger, Curtis~L. Janssen, Edward~T. Seidl, Wesley~D. Allen, Henry~F.
  Schaefer, Rollin~A. King, Edward~F. Valeev, C.~David Sherrill, and T.~Daniel
  Crawford.
\newblock Psi4: {A}n open-source ab initio electronic structure program.
\newblock {\em WIREs Comput. Mol. Sci.}, 2(4):556--565, 2012.

\bibitem{parrish2017psi4}
Robert~M. Parrish, Lori~A. Burns, Daniel G.~A. Smith, Andrew~C. Simmonett,
  A.~Eugene DePrince~III, Edward~G. Hohenstein, Ugur Bozkaya, Alexander~Yu
  Sokolov, Roberto Di~Remigio, Ryan~M. Richard, et~al.
\newblock Psi4 1.1: {A}n open-source electronic structure program emphasizing
  automation, advanced libraries, and interoperability.
\newblock {\em J. Chem. Theory Comput.}, 13(7):3185--3197, 2017.

\bibitem{gdml}
Stefan Chmiela, Alexandre Tkatchenko, Huziel~E. Sauceda, Igor Poltavsky,
  Kristof~T. Sch{\"u}tt, and Klaus-Robert M{\"u}ller.
\newblock Machine learning of accurate energy-conserving molecular force
  fields.
\newblock {\em Sci. Adv.}, 3(5):e1603015, 2017.

\bibitem{gonzalez1999}
Leticia Gonz{\'a}lez, Otilia M{\'o}, and Manuel Y{\'a}{\~n}ez.
\newblock Density functional theory study on ethanol dimers and cyclic ethanol
  trimers.
\newblock {\em J. Chem. Phys.}, 111(9):3855--3861, 1999.

\bibitem{durig1990torsional}
J.~R. Durig and R.~A. Larsen.
\newblock Torsional vibrations and barriers to internal rotation for ethanol
  and 2, 2, 2-trifluoroethanol.
\newblock {\em J. Mol. Struct.}, 238:195--222, 1990.

\bibitem{wassermann2010ethanol}
Tobias~N. Wassermann and Martin~A. Suhm.
\newblock Ethanol monomers and dimers revisited: {A} raman study of
  conformational preferences and argon nanocoating effects.
\newblock {\em J. Phys. Chem. A}, 114(32):8223--8233, 2010.

\bibitem{durig1975raman}
J.~R. Durig, W.~E. Bucy, C.~J. Wurrey, and L.~A. Carreira.
\newblock Raman spectra of gases. {XVI}. torsional transitions in ethanol and
  ethanethiol.
\newblock {\em J. Phys. Chem. A}, 79(10):988--993, 1975.

\bibitem{poggio2016visual}
Tomaso Poggio and Fabio Anselmi.
\newblock {\em Visual cortex and deep networks: learning invariant
  representations}.
\newblock MIT Press, 2016.

\bibitem{anselmi2016invariance}
Fabio Anselmi, Lorenzo Rosasco, and Tomaso Poggio.
\newblock On invariance and selectivity in representation learning.
\newblock {\em Inf. Inference}, 5(2):134--158, 2016.

\bibitem{sener2018multi}
Ozan Sener and Vladlen Koltun.
\newblock Multi-task learning as multi-objective optimization.
\newblock In {\em Adv. Neural. Inf. Process. Syst. 31}, pages 525--536, 2018.

\bibitem{Behler2007b}
J{\"{o}}rg Behler, S{\"{o}}nke Lorenz, and Karsten Reuter.
\newblock Representing molecule-surface interactions with symmetry-adapted
  neural networks.
\newblock {\em J. Chem. Phys.}, 127(1):14705, 2007.

\bibitem{Behler2011}
J{\"{o}}rg Behler.
\newblock Atom-centered symmetry functions for constructing high-dimensional
  neural network potentials.
\newblock {\em J. Chem. Phys.}, 134(7):74106, 2011.

\bibitem{montavon2012learning}
Gr{\'e}goire Montavon, Katja Hansen, Siamac Fazli, Matthias Rupp, Franziska
  Biegler, Andreas Ziehe, Alexandre Tkatchenko, Anatole~V Lilienfeld, and
  Klaus-Robert M{\"u}ller.
\newblock Learning invariant representations of molecules for atomization
  energy prediction.
\newblock In {\em Adv. Neural. Inf. Process. Syst. 25}, pages 440--448, 2012.

\bibitem{gdml2}
Stefan Chmiela, Huziel~E. Sauceda, Klaus-Robert M{\"u}ller, and Alexandre
  Tkatchenko.
\newblock Towards exact molecular dynamics simulations with machine-learned
  force fields.
\newblock {\em Nat. Commun.}, 9(1):3887, 2018.

\bibitem{frohlich2005optimal}
Holger Fr{\"o}hlich, J{\"o}rg~K Wegner, Florian Sieker, and Andreas Zell.
\newblock Optimal assignment kernels for attributed molecular graphs.
\newblock In {\em Proceedings of the 22nd international conference on Machine
  learning}, pages 225--232. ACM, 2005.

\bibitem{benoit2011}
Wei Jiang, David~J. Hardy, James~C. Phillips, Alexander~D. MacKerell, Klaus
  Schulten, and Benoît Roux.
\newblock High-performance scalable molecular dynamics simulations of a
  polarizable force field based on classical drude oscillators in namd.
\newblock {\em J. Phys. Chem. Lett.}, 2(2):87--92, 2011.

\bibitem{CHARMM1983}
Bernard~R. Brooks, Robert~E. Bruccoleri, Barry~D. Olafson, David~J. States,
  S.~Swaminathan, and Martin Karplus.
\newblock {CHARMM}: {A} program for macromolecular energy, minimization, and
  dynamics calculations.
\newblock {\em J. Comput. Chem.}, 4(2):187--217, 1983.

\bibitem{charmm2009}
Bernard~R Brooks, Charles~L Brooks~III, Alexander~D Mac{K}erell~Jr, Lennart
  Nilsson, Robert~J Petrella, Beno{\^\i}t Roux, Youngdo Won, Georgios
  Archontis, Christian Bartels, Stefan Boresch, et~al.
\newblock {CHARMM}: {T}he biomolecular simulation program.
\newblock {\em J. Comput. Chem.}, 30(10):1545--1614, 2009.

\bibitem{gromacs2005}
David Van Der~Spoel, Erik Lindahl, Berk Hess, Gerrit Groenhof, Alan~E. Mark,
  and Herman~JC Berendsen.
\newblock {GROMACS}: {F}ast, flexible, and free.
\newblock {\em J. Comput. Chem.}, 26(16):1701--1718, 2005.

\bibitem{de2017use}
Phil De~Luna, Jennifer Wei, Yoshua Bengio, Al{\'a}n Aspuru-Guzik, and Edward
  Sargent.
\newblock Use machine learning to find energy materials.
\newblock {\em Nature}, 552(7683):23, 2017.

\end{thebibliography}

